Contactless Oxygen Monitoring with Gated Transformer

With the increasing popularity of telehealth, it becomes critical to ensure that basic physiological signals can be monitored accurately at home, with minimal patient overhead. In this paper, we propose a contactless approach for monitoring patients' blood oxygen at home, simply by analyzing the radio signals in the room, without any wearable devices. We extract the patients' respiration from the radio signals that bounce off their bodies and devise a novel neural network that infers a patient's oxygen estimates from their breathing signal. Our model, called \emph{Gated BERT-UNet}, is designed to adapt to the patient's medical indices (e.g., gender, sleep stages). It has multiple predictive heads and selects the most suitable head via a gate controlled by the person's physiological indices. Extensive empirical results show that our model achieves high accuracy on both medical and radio datasets.

==> source/fig/fig_breathing_new.tex <==
% \begin{figure*}[h!]
% \begin{tabular}{@{\hspace{0mm}}c}
% \includegraphics[width=1\columnwidth]{./figures/appendix/breathing_whole_night.png} \\
% Whole night \\
% \includegraphics[width=1\columnwidth]{./figures/appendix/breathing_zoom_in.png} \\
% Close-up 
% \end{tabular}
% \vspace{-4mm}
% \caption{\yc{Visualization of raw breathing signal, its spectrum, breathing rate and the corresponding oxygen saturation. }}
% \end{figure*}

\begin{figure}[h!]
\centering
\begin{tabular}{@{\hspace{0mm}}c}
\includegraphics[width=0.8\columnwidth]{./figures/appendix/breathing_case_1.pdf} \\
(a) Normal Breathing  \\
\includegraphics[width=0.8\columnwidth]{./figures/appendix/breathing_case_4.pdf} \\
(b) Abnormal Breathing \\
\includegraphics[width=0.8\columnwidth]{./figures/appendix/breathing_case_2.pdf} \\
(c) Abnormal Breathing \\
\includegraphics[width=0.8\columnwidth]{./figures/appendix/breathing_case_5.pdf} \\
(d) Abnormal Breathing \\
\end{tabular}
% \vspace{-4mm}
\caption{
Visualization of several breathing signals and their corresponding predicted oxygen saturation. (a) is an example of normal breathing signals. (b-d) are examples of different abnormal breathing signals. In every figure, the first row shows the breathing signals while the second row shows the ground truth oxygen saturation (in blue) and the oxygen saturation predicted by our GNP model (in orange).}\label{fig:breathing}
\end{figure}
% \vspace{-2mm}

==> source/fig/fig_breathing_rate_vs_full_breathing.tex <==
% \begin{figure*}[h!]
% \begin{tabular}{@{\hspace{0mm}}c}
% \includegraphics[width=1\columnwidth]{./figures/appendix/breathing_whole_night.png} \\
% Whole night \\
% \includegraphics[width=1\columnwidth]{./figures/appendix/breathing_zoom_in.png} \\
% Close-up 
% \end{tabular}
% \vspace{-4mm}
% \caption{\yc{Visualization of raw breathing signal, its spectrum, breathing rate and the corresponding oxygen saturation. }}
% \end{figure*}

\begin{figure*}[htb]
\centering
\begin{tabular}{@{\hspace{0mm}}c@{\hspace{0mm}}c@{\hspace{0mm}}c}
\includegraphics[width=0.33\textwidth]{./figures/experiments/breathing_rate_1.pdf} &
\includegraphics[width=0.33\textwidth]{./figures/experiments/breathing_rate_2.pdf} &
\includegraphics[width=0.33\textwidth]{./figures/experiments/breathing_rate_3.pdf} \\
(a) & (b) & (c) \\
% \includegraphics[width=0.49\textwidth]{./figures/appendix/breathing_rate_vs_full_breathing_4.png} \\
% (c) & (d) \\
\end{tabular}
\vspace{-4mm}
\caption{
% \yy{Comparison of the breathing signals and the breathing rates in containing the information about oxygen saturation. Here are examples of three pairs of subjects who have different oxygen saturation. Their breathing rates are quite similar and less informative to infer the correct oxygen. Compared to the breathing rate, the breathing signals are much more informative and correlated to the oxygen. Our model can capture the shape difference of breathing signals and make the correct oxygen prediction.}
Demonstrations of breathing signals being more discriminative than breathing rate for oxygen saturation prediction. (a)(b)(c) show three examples where two subjects have similar breathing rates but very different oxygen levels. While subjects' breathing signals are more correlated to the oxygenation. Based on breathing signals, our model make accurate predictions of oxygen saturation.
}\label{fig:breathing_rate}
\end{figure*}


==> source/fig/fig_example.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.6\columnwidth]{./figures/method/eg_signals.pdf}\\
%\vspace{-1mm}(a)\\
%\vspace{2mm}
%\includegraphics[width=1.0\columnwidth]{./figures/method/overview.pdf}
%(b)
\vspace{-2mm}
\caption{Breathing signal and corresponding SpO2 signal.}
\label{fig:eg-br-oxy}
\end{figure}


==> source/fig/fig_example_wrap.tex <==
% \begin{wrapfigure}{r}{0.6\textwidth}
% \centering
% \vspace{-5mm}
% \includegraphics[width=0.6\columnwidth]{./figures/method/eg_signals.pdf}
% \vspace{-7mm}
% \caption{Breathing signal and corresponding SpO2 signal.}
% \vspace{-5mm}
% \label{fig:eg-br-oxy}
% \end{wrapfigure}


==> source/fig/fig_visualize_rf_pred.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.95\columnwidth]{figures/experiments/mgh1.pdf}\\
\vspace{-3mm}
\caption{Example of SpO2 prediction results on RF dataset.}
\vspace{-3mm}
\label{fig:visualize_rf}
\end{figure}


==> source/fig/sidebyside_race_visrf.tex <==
\begin{figure}[t!]
  \begin{minipage}{.6\linewidth}
    \centering
        \includegraphics[width=0.9\textwidth]{figures/experiments/mgh1.pdf}\\
        \vspace{-4mm}
        \caption{Example of SpO2 prediction results on RF dataset.}
        \label{fig:visualize_rf}
  \end{minipage}
    \hfill
  \begin{minipage}{.38\linewidth}
    \centering
        \includegraphics[width=0.95\textwidth]{./figures/experiments/races_results_new.pdf}
        \vspace{-1mm}
        \caption{Box plots of ground-truth oxygen saturation and our prediction for two races.} 
        \label{fig:race-result}
  \end{minipage}%
  \vspace{-5mm}
\end{figure}
% \vspace{-10mm}


==> source/old/abstract.tex <==
\begin{abstract}
With the increasing popularity of telehealth and remote health monitoring, it becomes critical to ensure that basic physiological signals can be monitored accurately at home, with minimal patient overhead. In this paper, we introduce \SYSTEMNAME, a system that monitors patients' blood oxygen at home simply by analyzing the radio signals in the room, without any wearable devices. We extract the patients' respiration from the radio signals that bounce off their body, and devise a novel neural network that infers a patient's oxygen measurements from their breathing signal. Motivated by personalized medicine, we design our neural network to adapt to the patient's  medical indices (e.g., gender, smoking status) and leverage them for improved performance. Our model, which we refer to as \emph{Gated Neural Predictor}, has multiple predictive sub-networks. It selects the most suitable sub-network via a gate controlled by the subject's physiological indices. Experimental results demonstrate that our model achieves high accuracy on medical and radio-frequency datasets. 
\end{abstract}

==> source/old/exp.tex <==
\section{Experiments}
\label{sec:exp}
We present the results of empirical evaluation on medical datasets and RF data. For the error metric, we use the average absolute error between the predicted oxygen saturation $\hat{y}$ and the ground-truth $y$ at any point in time. The error is first averaged for every night and each subject, i.e., $\frac{1}{T} \sum_{t=1}^T \|y^t - \hat{y}^t\|$. We then report the mean and standard deviation of per-night averaged errors of the dataset.


\input{source/exp_dataset}


\subsection{Compared Models}
\label{sec:models}
We would like to evaluate both our backbone \textit{BERT-UNet} architecture, and our \textit{GNP} design for incorporating physiological variables. 

To evaluate our backbone design without side variables, we compare our \textit{BERT-UNet} model to prior models for learning from physiological signals.   Specifically, we compare the following models: (a) \textit{Linear Regression}: we use six hand-crafted time series statistics proposed by \cite{picard2001toward} as breathing features and run linear regression. (b) \textit{CNN-RNN}: we adapt the CNN-RNN proposed in \cite{zhao2017learning} to our oxygen prediction task. It contains a feature encoder (CNN-RNN) and an oxygen predictor. (c) \textit{BERT-UNet}: our backbone model described in \ref{model:basemodel}. 


To evaluate our design for incorporating side information, we compare the following models:
(a) Our \textit{Gated Neural Predictor (GNP)} model which uses a multi-head model gated by physiological variables. 
% Unless stated otherwise GNP uses 6 heads (i.e., 6 states) and assigns categories to heads according to the gradient as described in Sec.~\ref{sec:xxx}.
(b) \textit{VarAug}: This model uses BERT-UNet as backbone and takes accessible variables as extra inputs and inaccessible variables as auxiliary tasks. (c) \textit{PCGrad-Adapted}: we adapt the PCGrad~\cite{PCGrad} to our task. The original PCGrad was proposed for improving multi-task learning and deal with scenarios where the tasks have divergent gradients. The model shares one encoder across different tasks, and projects the divergent gradients along consistent directions during training. To adapt this design to our task we augment the BERT-UNet model with PCGrad applied to subgroups with different values for their medical indices.  To train the single predictor $F$, in each iteration, we compute losses on different subgroups. Each subgroup $i$ has an oxygen prediction loss $\gL_i$. We compute the predictor's gradients $\nabla_{\theta_f} \gL_i$ for each loss, and calibrate them by PCGrad. We then use the calibrated gradients to update the parameters of the predictor.

% \hh{
% Our experiments focus on using sleep stages and gender as side variables due to their accessibility and close relationships to oxygen. See \secref{sec:grad} for more details about the variables and how we group different sleep stages and gender for our GNP model. 
% }

% \subsection{Models} 
% As we describe in \Secref{sec:method}, our models focus on predicting oxygen from breathing while leveraging auxiliary gender and sleep stage information. We evaluate the following models: (a) \textit{Single-Headed}: the vanilla backbone model. (b) \textit{Multi-Task}: the model that takes gender as an extra input and is trained with sleep stages as an auxiliary task. (c) \textit{Multi-Headed}: the model that uses multiple heads to predict oxygen level for different switch status.  (d) We also compare with an adaptation of the Projecting Conflicting Gradient \textit{PCGrad-Adapted}. The original PCGrad was proposed for improved multi-task learning to deal with scenarios where the various tasks have divergent gradients~\citep{PCGrad}.  In that case, PCGrad projects the divergent gradients along consistent directions. In our context, the gradients of the tasks themselves -- i.e., oxygen prediction and sleep stage prediction -- do not diverge. Hence, simply applying PCGrad to our problem should be no different from the Multi-Task model. However, we can adapt PCGrad to be more suitable for our problem. In our case, the gradients of subgroups (i.e., subjects with different status) in the input data with respect to the main task can be divergent or significantly different.  We can think of learning a mapping from breathing to oxygen for different subject status as different sub-tasks. Then, we can augment our backbone model with PCGrad applied to these sub-tasks. Specifically, to train the single predictor $F$,  We compute 6 different losses based on the six subject status corresponding to our 6-headed model. For each subject status $i$, we have an oxygen prediction loss $\gL_{o}^i$ for that status. Mathematically, $\gL_{o}^i(F,E) = (\sum_{t: S^t=i} 1)^{-1} \sum_{t: S^t=i} |F(E(x_b))^t - y^t|$. We compute the predictor's gradients $\nabla_{\theta_f} \gL_{o}^{i}$ for each loss and update the predictor by the gradient calibrated by PCGrad.

\input{source/fig/visualize_shhs}

\input{source/table/main-result-v5}

\subsection{Evaluation on Medical Datasets}
We empirically evaluate the models in Sec.~\ref{sec:models} on the medical datasets.  All models are trained on the union of the training sets from the three medical datasets, and tested on each test set, and on the union of the three test sets. For models that incorporate side variables, we use gender as the accessible variable and sleep stages as the inaccessible variable. In GNP, we use the gradient to pick gate status as described in Sec.~\ref{sec:grad-sim}, which results in the following categories: (male, awake), (male, REM), (male, N1+N2+N3), (female, awake), (female, REM), (female, N1+N2+N3). The sleep stages themselves are learned from the input since they are an inaccessible variable. In the baselines, the gender variable is provided as an additional input and the sleep stages are used as an auxiliary task in a multitask model. 


\textbf{Results.}
The results are shown in \Tabref{tab:res-main}. The upper rows in the table show the results of models that do not leverage side variables.   The table shows that the BERT-UNet model has an average prediction error of 1.62\%, and consistently outperforms the linear regression model and the CNN-RNN model on all datasets. 

The bottom rows in the table show the results of models leveraging accessible and inaccessible medical variables. VarAug, PCGrad, and our GNP are all built using our BERT-UNet architecture. The objective is to compare their ability to leverage side variables.  The table shows that VarAug, PCGrad, and GNP have an overall average prediction error of 1.58\%, 1.69\%, and 1.55\%, respectively. VarAug and the GNP perform better than the backbone BERT-UNet demonstrating the benefit of leveraging side variables. PCGrad performs worse than the backbone BERT-UNet showing that design could not utilize the side variables effectively. Our GNP outperforms both baselines on all three datasets, demonstrating that a gated multi-head approach works best for such categorical side variables. More generally, these results show for the first time that respiration signals can be used to infer oxygen saturation. Further, the errors are comparable to the accuracy of consumer pulse oximeters (wearable devices with an average error ranges from 0.4\% to 3.5\% ~\citep{lipnick2016accuracy}).

\textbf{Visualization.}
To better understand how the model works, we visualize an example of its prediction. 
Figure~\ref{fig:visualize_shhs2} visualizes the predicted oxygen saturation of the GNP model and the VarAug model on a male subject in the SHHS dataset. As the ground-truth oxygen saturation are integers, we rounded the predicted oxygen values. The background color indicates different sleep stages. The `light grey' and `white' corresponds to `REM' and `Awake', respectively. For clarity, we use one color `dark grey' for all three non-REM `Sleep' stages, N1, N2, and N3. We observe that GNP consistently outperforms VarAug over the whole night. The small panel focus on different sleep stages. In general, different sleep stages tend to show different behavior and hence the importance of using a gated model. Specifically, oxygen is typically more stable during non-REM `Sleep' than REM and Awake stages.  The figures shows that GNP can track the ups and downs in oxygen and is significantly more accurate than VarAug. This experiment demonstrates that the way we incorporate the sleep stages into the model improves performance across different sleep stages. Please see the supplement for visualizations on the other datasets.

% Figure~\ref{fig:visualize_shhs2} visualizes the predicted oxygen saturation of the Multi-Headed model and the Multi-Task model on a male subject in the SHHS dataset. As the ground-truth oxygen saturation are integers, we rounded the predicted oxygen saturation into integers. The background color indicates different sleep stages. The `light grey' and `white' corresponds to `REM' and `Awake', respectively. For clarity, we use one color `dark grey' for all three non-REM `Sleep' stages, N1, N2, and N3. We observe that the Multi-Headed model consistently performs better than the Multi-Task model over the whole night. In non-REM `Sleep', the ground-truth oxygen saturation is more stable. The Multi-Headed model predicts more accurate oxygen than the Multi-Task model. In the `REM' stage, people usually have lower oxygen saturation with larger variance. The Multi-Headed model predicts the ups and downs and captures the changes in blood oxygen. In the `Awake' stage, the Multi-Headed model predicts the more dramatic changes, while the Multi-Task model has a larger bias. This experiment demonstrates that the way we incorporate the sleep stages into the model improves the performance across different sleep stages. 
% Please refer to \Secref{sec:visual} for more prediciton visualizations.

\input{source/fig/fig_breathing_rate_vs_full_breathing}

\subsection{Evaluation on RF Dataset}
As mentioned earlier, the RF dataset is not large enough to train the model on RF signals. Hence, we train our model to infer oxygen from respiration signals. We then test the model directly on RF signals. Specifically, we  evaluate the GNP model on the RF dataset. We test the model on both RF-based respiration signals and the corresponding breathing signals measured by a breathing belt. The results are shown in \Tabref{tab:umass}. We observe that the model works well on the
RF dataset with a small prediction error, no matter which breathing signal is used. The prediction error of using the RF-respiration signals ($1.28\%$) is even slightly lower than using the respiration signals from the breathing belt ($1.30\%$). This is because the noise in the respiration measured using RF signal is different from the noise in the breathing belt measurements. The noise in the RF-based measurements tends to increase with motion, and hence we see that the model prediction error is higher for the awake stage. In contrast, the error in the breathing belt depends on the sleep posture and the positioning of the belt on the body. Also, comparing with the error from the previous section, we find the model is performing better on the RF dataset than on the medical datasets, i.e., $1.30\%$ vs. $1.55\%$. We believe the reason is that the RF dataset is collected with healthy individuals and hence has less complexity and is easier to predict. These results show the first demonstration of predicting oxygen saturation from radio signals without any body contact.
% \vspace{-4mm}
\input{source/table/umass-result}
% \vspace{-4mm}
% In this section, we evaluate whether our model, which is trained on respiration measured using a breathing belt, can generalize to predicting oxygen from respiration signals measured via radio waves. We directly apply a Multi-Headed model trained on the BB-respiration signals in medical datasets, to the RF dataset. For comparison, we test the model on both RF-respiration signals and BB-respiration signals from the RF dataset. The results are shown in \Tabref{tab:umass}. We observe that the model works well on RF dataset with a small prediction error, no matter which breathing signal is used. The prediction error of using the RF-respiration signals ($1.28\%$) is even slightly lower than using the BB-respiration signals ($1.30\%$). This is because the noise in the respiration measured using RF signal is different from the noise in the breathing belt measurements. The noise in the RF-based measurements tend to increase with motion and hence we see that the model prediction error is higher for the aware stage. In contrast, the error in the breathing belt depends on the sleep posture and the positioning of the belt on the body. Also, comparing with the error from previous section, we find the model is performing better on the RF dataset than on the medical datasets, i.e., $1.30\%$ vs. $1.62\%$. We believe the reason is that the RF dataset is collected with healthy individuals and hence has less complexity and is easier to predict. These results show the first demonstration of predicting oxygen saturation from radio signals without any body contact.

\subsection{Results for Different Skin Colors}
\input{source/fig/race_result}

% \textbf{Error Analysis and Relation to Skin Color.}
One important issue to keep in mind is that our model learns from ground-truth oxygen saturation measured using pulse oximeters (today oximetry is the only way for continuous noninvasive monitoring of blood oxygen). Hence, to understand the prediction errors and their potential causes, we plot in \Figref{fig:race-result} the distributions of the ground-truth oxygen and the GNP predicted oxygen for different races, for all datasets. Interestingly, the ground-truth measurements from oximetry show a clear discrepancy between black and white subjects. In particular, they show that black subjects have higher blood oxygen. This is compatible with past findings that pulse oximeter overestimates blood oxygen in dark-skinned subjects~\citep{feiner2007dark}. In contrast, our model predictions show much more similar oxygen distributions for the two races. It is interesting that while the model learned from what seems to be biased ground-truth, the results show that the model is able to correct, to some extent, for this bias. Admittedly, these observations are inductive since there is no way to measure the exact errors in the ground-truth labels. 

% One important issue to keep in mind is that our model learns from ground-truth data measured using pulse oximeters (today oximetry is the only way for continuous noninvasive monitoring of blood oxygen). Hence, to understand the prediction errors and their potential causes, we plot in \Figref{fig:race-result} the distributions of the ground-truth SpO2 and the predicted SpO2 by the Multi-Headed model for different races, for all datasets. Interestingly,  the ground-truth SpO2 from oximetry shows a clear discrepancy between black and white subjects. In particular, the ground-truth oxygen distributions show that black subjects have higher blood oxygen. This is compatible with past findings that pulse oximeter overestimates blood oxygen in dark-skinned subjects~\citep{feiner2007dark}. In contrast, the model prediction shows much more similar oxygen distributions for the two races. It is interesting that while the model learned from what seems to be biased ground-truth, the results show that the model is able to correct, to some extent, for this bias. Admittedly, these observations are inductive since there is no way to measure the exact errors in the ground-truth labels. 

The distributions in \Figref{fig:race-result} also show that the model tends to miss the very high and very low oxygen values. This is expected given that only a very small percentage of the ground-truth data falls in the tails. One would expect that the performance on very high and very low values would improve if there is sufficient training data in those ranges. 

\vspace{-0.1in}
\subsection{Breathing Signals vs. Breathing Rate} 
It is important to note that we use the breathing signals instead of the breathing rates. Breathing signals contain richer information about oxygen saturation than the breathing rate. Figure \ref{fig:breathing_rate} shows several pairs of subjects who have the same breathing rate but quite different oxygen saturation values. It also shows that our model is able to predict the correct oxygen levels and is not confused by the fact that the subjects have the same breathing rates.


% \subsection{Ablation Study}
% \yy{We study several backbone models with different architecture on the SHHS dataset. (a) \textit{FCN}: It contains only the encoder, which shrink the output by 10 times of the input dimension. (b) \textit{UNet}: it contains an encoder which consists of a fully convolution network and a predictor that consists of several De-convolution layers, which up-samples the extracted features to the same time resolution of oxygen saturation. It dose not contain any temporal models. (c) \textit{LSTM-UNet}: it has the same encoder and decoder with the UNet, but adds a LSTM layer at the bottleneck of the UNet. (d) \textit{Bi-LSTM-UNet}: it adds a bi-directional LSTM layer at the bottleneck of the UNet. (e) \textit{BERT-UNet}: our strong backbone model, which has a BERT model at the bottleneck of the UNet. 
% We also investigate two naive base models, i.e., \textit{Linear Regression} and \textit{Random Forest Regression}. To extract the hand-crafted features from respiration signals, we use the six statistical time series feature suggested by~\citep{picard2001toward}.}

% \begin{table*}[htb]
% \centering
% \caption{\yc{Ablation study of our model.}}
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \toprule
% Method & Linear Regression & Random Forest & FCN & UNet & LSTM-UNet & Bi-LSTM-UNet & Bert-UNet \\ \hline 
% Prediction Error & 1.86 $\pm$ 1.72 & 1.85 $\pm$ 1.73 & 1.86 $\pm$ 1.69 &  &  &  & \\
% \bottomrule
% \end{tabular}
% \end{table*}
\vspace{-0.1in}
\subsection{Analysis of Physiological Variables}\label{sec:exp_diff_var}
We further study the benefits of a gated model for incorporating side information from different variables. We conduct experiments on the SHHS dataset since it has a rich collection of  medical indices. For every single variable we choose, we compare the GNP model with VarAug. Recall that the only difference between these two models is in the way they leverage categorical variables. Table \ref{tab:diff_var} shows the comparison regarding Sleep Stage (awake vs. REM vs. Sleep), Gender (male vs. female), Smoke States (non-smoker vs. smoker), Asthma (having Asthma or not) and Aspirin (taking aspirin or not). The result shows that our model consistently outperforms VarAug, indicating that GNP is a better solution to deal with discontinuous physiological variables. This supports our theoretical analysis in Sec.~\ref{sec:theory}.  We believe the applicability of this result extend beyond the specific task of oxygen prediction to other tasks that involve adaptation to categorical or binary variables. As a reference, the first row in \tabref{tab:diff_var} shows the error with no variables, i.e., the errors of the backbone BERT-UNET model. Note that the errors in \tabref{tab:diff_var} are larger than BERT-UNet's errors shown in \tabref{tab:res-main}. This is because the models here are trained on the SHHS dataset while in the models in 
\tabref{tab:res-main} are trained on the three datasets combined.

\vspace{-4mm}
\input{source/table/diff_variables}
\vspace{-1mm}
%\input{source/exp-grad}


==> source/old/exp_dataset.tex <==
\subsection{Datasets} \label{sec:datasets}
% \input{source/table/dataset}

\hh{\Tabref{tab:dataset} summarizes the statistics of datasets used in our experiments. SHHS, MESA, MrOS refer to the three public medical datasets: Sleep Heart Health Study~\citep{SHHS2}, Multi-Ethnic Study of Atherosclerosis~\citep{MESA}, and Osteoporotic Fractures in Men Study~\citep{MROS} developed for sleep study. They are large datasets containing thousands of subjects with different gender, age, health conditions. We train our model on the union of these three datasets. We randomly split the data such that 70\% of the subjects are used for training while the rest 30\% of subjects are reserved for testing. We also collected a small dataset using our radio device to validate our system in the real application of contactless oxygen monitoring. 
}

\noindent \textbf{Medical Datasets.} 
\hh{The medical datasets contain rich physiological indices of the subjects. We mainly use the following during our experiments: 1) Respiration signals measured by breathing belt; 2) Oxygenation measured by pulse oximetry; 3) Sleep stage which indicates the stage of the subject during sleep. There are five stages: Awake, Rapid Eye Movement (REM) and three different levels of sleep~(N1, N2, and N3).
We note that the subjects in these studies have an wide age range and suffer from a variety of diseases such as chronic bronchitis, cardiovascular diseases, and diabetes. This allows for a wider range of oxygen variability beyond the typical range of healthy individuals.  
}

%  (`Awake', `Rapid Eye Movement (REM)', `N1', `N2', and `N3')

% We leverage three publicly-available medical datasets: Sleep Heart Health Study (\textit{SHHS})~\citep{SHHS2}, Multi-Ethnic Study of Atherosclerosis (\textit{MESA})~\citep{MESA}, and Osteoporotic Fractures in Men Study (\textit{MrOS})~\citep{MROS}. The first two datasets have males and females, whereas the last one has male subjects. 
% These datasets are collected during sleep studies. For each subject, they include the respiration signal throughout the night along with the corresponding oxygen time series. They also contain a variety of side variables including sleep stages, which for every time instance assign to the subject one of the following: Awake, Rapid Eye Movement (REM) or one of three non-REM stages N1, N2, and N3.
% SHHS, MESA, and MrOS contains 2651, 2056, and 1026 subjects, respectively. We randomly split the training and testing sets for SHHS, MESA, and MrOS as 1855/796, 1439/617, and 718/308, and keep the same splits in all experiments. 
\begin{figure}[t!]
\centering
\includegraphics[width=0.6\columnwidth]{./figures/method/RF_Device.pdf}
\vspace{-2mm}
\caption{Radio device used to collect RF signals. The monitoring is done in a contactless manner and without imposing any overhead on the patient. }
\vspace{-4mm}
\label{fig:radio}
\end{figure}

% \vspace{-4mm}

\noindent \textbf{RF Dataset.}
% We collect a small dataset that contains both radio signals and oxygen saturation.  The dataset is collected in a sleep lab  and contains 31 nights of data from 14 individuals. All subjects in this study are healthy.  Each subject is monitored using the standard sleep channels as in the medical datasets above (oxygen saturation, respiration belts, sleep stages, etc.). Additionally, a radio device is installed in the room to collect RF signals. The radio shown in Fig.~\ref{fig:radio} uses a standard technology widely adopted in past work on health monitoring using radio signals~\cite{yue2018extracting,hsu2017zero,zhao2017learning}. The radio signals are processed with the algorithm in~\cite{adib2015smart} to extract the subject's breathing. Thus, this dataset contains for each subject their breathing signal as inferred from radio waves, their breathing signals measured using a breathing belt, and their oxygen level measured using pulse oximetery. 
\red{We collect a small RF dataset from the sleep labs of a university and a hospital. It contains 49 nights of data from 32 subjects. 
\Figref{fig:radio} shows an example data collection setting: 
a radio device is installed in the room to collect RF signals; The subject is asked to wear pulse oximetery that record containing oxygen saturation data during the sleep. As we mentioned in the method section, the radio signals are processed to extract the subject's respiration signals. We later synchronize the respiration signals and oxygenation data and build the RF dataset.
% The radio shown in Fig.~\ref{fig:radio} uses a standard technology widely adopted in past work on health monitoring using radio signals~\cite{yue2018extracting,hsu2017zero,zhao2017learning}. The radio signals are processed with the algorithm in~\cite{adib2015smart} to extract the subject's breathing. For each night of each subject, the data includes their breathing signal inferred from radio waves, and their corresponding ground truth blood oxygen saturation.
}

==> source/old/related.tex <==
\section{Related Work}

% NOTE:
\noindent \textbf{Contactless Health Sensing with Radio Signals} The past decade has seen a rapid growth in research on passive sensing using radio frequency (RF) signals. Early work has demonstrated the possibility of sensing one's breathing and heart rate using radio signals~\citep{adib2015smart}. Building on this work, researchers have found that by carefully analyzing the RF signals that bounce off the human body, they can monitor a variety of health metrics including sleep, respiration signal, heart rate, gait, falls, and even human emotions~\citep{nguyen2016continuous,wang2017tensorbeat,yue2018extracting, wigait,wifall,rf-fall,eq-radio,jiang2018smart}. Our work adds a new method to the general area of contactless sensing of physiological signals from radio waves. 

\noindent \textbf{Predicting Oxygen Saturation}
No past work predicts oxygen levels from breathing signals or radio waves. Past work on oxygen prediction focuses on extrapolating or interpolating oxygen measurements. Specifically, several papers use auto-regressive models that take past oxygen readings and extrapolate oxygen level for the next few minutes~\citep{elmoaqet2013predicting,elmoaqet2014novel,elmoaqet2016multi}. Other work uses current oxygen measurements to predict changes in oxygen in the five minutes after adjusting ventilator setting~\citep{ghazal2019using}. Some past work models the photoplethysmogram (PPG) signal, i.e., the raw data used by pulse oximeters. For example, \citep{martin2013stochastic} proposes a stochastic model of PPG that reconstructs missing oxygen readings from observed values. Thus, all past methods estimate future or missing oxygen values from available oxygen measurements. Our work differs from all of this prior work in that we predict oxygen values from other modalities like respiration or radio waves, and enable oxygen sensing in a contactless manner.
% Our work differs from these methods in that it predicts oxygen without requiring access to any oxygen measurements. Also, we predict oxygen from different signals like respiration or radio waves. 


\noindent \textbf{Adaptation of Machine Learning Models to Medical Indices}
Prior deep learning models operating on physiological signals typically do not adapt to a person's medical indices. For example, the literature has models that infer sleep stages from respiration~\citep{zhao2017learning}, detect arrhythmia from ECG~\citep{kiyasseh2020clocs,kiyasseh2020clops}, and classify emotion from EEG signals~\citep{murugappan2010classification}. A recent survey~\citep{rim2020deep} collected 147 papers about learning with physiological signals. None of the deep models therein adapts to a person's medical indices. 

%TODO
The deep learning literature includes a few approaches for leveraging auxiliary variables. If the variable is available at inference time, past work typically takes it as an extra input feature~\cite{narayan2017neural,shen2016automatic}. Some variables are only accessible during training. In this case, they are typically used as an extra supervisor to regularize the model via multi-task learning~\cite{liu2019auxiliary,mordan2018revisiting,valada2018deep}. 
% In Sec.~\ref{sec:exp_diff_var}, 
We analytically and empirically show that GNP is a better design for adapting to categorical variables, and outperforms methods that take variables as input and those that leverage them through multitask learning. 
% \sout{There are also deep models that leverage side variables to adapt the convolution kernel~\citep{kang2020incorporating,choi2019adaptive,liu2019context}. Such methods however do not apply to our task since they cannot adapt to dense auxiliary signals (e.g., sleep stages). }

%However, their mode of adaptation is different from ours since they typically adapt to continuous variables like camera height and orientation or some similarity distance~\citep{kang2020incorporating,narayan2017neural,valada2018deep}. 

==> source/sup_race.tex <==
\newpage

\subsection{Results for Different Skin Colors}

Since pulse oximeters rely on measuring light absorbance through the finger, they are known affected by skin color and tend to overestimate blood oxygen saturation in subjects with dark skin~\cite{feiner2007dark,sjoding2020racial}. This issue was also the topic of a recent news outbreak after a large study that looked at tens of thousands of white and black COVID patients found that the ``reliance on pulse oximetry to triage patients and adjust supplemental oxygen levels may place black patients at increased risk for hypoxaemia"~\cite{sjoding2020racial}. 

In contrast, since neither breathing nor RF signals is affected by skin color, a model that estimates oxygen saturation from breathing or RF signals has no intrinsic bias against skin color. 
% Unfortunately however there is still some bias since we are training our model with ground truth data obtained from pulse oximeters. The hope however is that the bias in our model is smaller since the model is not told explicitly about the subjects' skin color. 
Hence as it trains, it tries to learn a general mapping that fits all skin colors. 
To understand the prediction errors and their relation to skin color, we plot in \Figref{fig:race-result} the distributions of the ground-truth oxygen and the GNP predicted oxygen for different races, for the union of all datasets. Interestingly, the ground-truth measurements from oximetry show a clear discrepancy between black and white subjects. In particular, they show that black subjects have higher average blood oxygen. This is compatible with past findings that pulse oximeter overestimates blood oxygen in dark-skinned subjects~\cite{feiner2007dark}. In contrast, our model kind of corrects or reduces the bias -- the predictions reduce the average oxygen saturation for the black subjects and show much more similar oxygen distributions for the two races. 
% It is interesting that while the model learned from what seems to be a biased ground-truth, the results show that the model is less biased than pulse oximetry. As explained above this is because the learning process makes the neural network search for the best model to map breathing to oxygen, independent of skin color.  
 
%  The distributions in \Figref{fig:race-result} also show that the model tends to miss the very high and very low oxygen values. This is expected given that only a very small percentage of the ground-truth data falls in the tails. One would expect that the performance on very high and very low values would improve if there were sufficient training data in those ranges. 

\input{source/fig/race_result}

==> source/table/dataset.tex <==
\begin{table}[ht]\small
\caption{Datasets Statistics} \label{tab:dataset}
\centering
\begin{tabular}{c|ccc|c}
\toprule
Dataset & SHHS & MESA & MrOS & Our RF \\ \hline
Number of subjects & 2651 & 2056 & 1026 & 32 \\
Length of data (hours) & & & \\
Percentage of males (\%) & 46 & 54 & 100 & \\
Age Range & [44,90] & [54,95] & [67,90] & \\
\bottomrule
\end{tabular}
% \vspace{-5mm}
\end{table}

==> source/table/diff_variables.tex <==
\begin{table}[ht]\small
\caption{
Errors of the VarAug model and our GNP model using different variables. \textbf{Results are on the SHHS dataset.} 
} \label{tab:diff_var}
\centering
\begin{tabular}{c|cc}
\toprule
% Variable & VarAsInput & VarAsOutpu & GNP   (Ours) \\ \hline
% stage & 1.66 $\pm$ 1.60 & 1.744 & 1.719 \\
% gender & 1.756 & 1.752 & 1.719 \\
% bmi & 1.732 & 1.762 & 1.74 \\
% smoke & 1.737 & 1.758 & 1.735 \\
% aspirin & 1.749 & 1.761 & 1.725 \\
% education & 1.747 & 1.777 & 1.732 \\
% asthma & 1.763 & 1.751 & 1.735 \\
% height & 1.736 & 1.868 & 1.742 \\
Variable & BERT-UNet+VarAug & BERT-UNet+GNP \\ \hline
None & 1.73 $\pm$ 1.58 & - \\ \hline
Sleep Stage & 1.69 $\pm$ 1.60 & 1.66 $\pm$ 1.54 \\
% BMI & 1.68 $\pm$ 1.58 & 1.65 $\pm$ 1.55 \\
Gender & 1.69 $\pm$ 1.57 & 1.64 $\pm$ 1.55 \\
Smoke & 1.67 $\pm$ 1.52 & 1.65 $\pm$ 1.53 \\
Asthema & 1.70 $\pm$ 1.58 & 1.67 $\pm$ 1.54 \\
Aspirin & 1.70 $\pm$ 1.56 & 1.66 $\pm$ 1.54 \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

==> source/table/main-result-v5.tex <==
% \begin{table*}[] 
% \caption{\yy{Prediction error (mean $\pm$ std) of different models trained on all three medical datasets and test on each dataset and the overall datasets.} }
% \label{tab:res-main}
% % \footnotesize
% \centering
% \begin{tabular}{c|c||c|c|c||c} 
% \toprule
% & Model       & {SHHS} & {MESA} & {MrOS} & Overall\\ \hline
% % \yc{Linear Regression} & \yc{1.86 $\pm$ 1.72} & \yc{1.73 $\pm$ 1.73} & \yc{1.87 $\pm$ 1.69} & \yc{1.81 $\pm$ 1.72} \\
% % \yc{Random Forest} & \yc{1.85 $\pm$ 1.73} & \yc{1.72 $\pm$ 1.73} & \yc{1.89 $\pm$ 1.71 }& \yc{1.81 $\pm$ 1.73 }\\
% & Linear Regression & 1.86 $\pm$ 1.72 & 1.73 $\pm$ 1.73 & 1.87 $\pm$ 1.69 & 1.81 $\pm$ 1.72 \\
% % Random Forest & 1.85 $\pm$ 1.73 & 1.72 $\pm$ 1.73 & 1.89 $\pm$ 1.71 & 1.81 $\pm$ 1.73 \\
% w/o Physiological Variables & CNN-RNN & - & - & - & - \\
% & \textbf{BERT-UNet (Ours)} & \textbf{1.68} $\pm$ \textbf{1.56}  & \textbf{1.59} $\pm$ \textbf{1.58} &  \textbf{1.76} $\pm$ \textbf{1.56} & \textbf{1.66} $\pm$ \textbf{1.53}\\ \hline
% & \yy{BERT-UNet + VarAug} &  1.69 $\pm$ 1.57 & 1.51 $\pm$ 1.56 &  1.71 $\pm$ 1.57 & 1.62 $\pm$ 1.53  \\
% w Physiological Variables & \yy{BERT-UNet + PCGrad} & 1.74 $\pm$ 1.58   &  1.62 $\pm$ 1.57 & 1.74 $\pm$ 1.53 & 1.71 $\pm$ 1.54 \\
% & \yy{\textbf{BERT-UNet + GNP (Ours)}}  & \textbf{1.62 $\pm$ 1.54} & \textbf{1.48 $\pm$ 1.51} & \textbf{1.66 $\pm$ 1.51} & \textbf{1.58 $\pm$ 1.49}\\
% % \yy{CNN-RNN + GNP}  & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[ht]
\centering
\caption{Prediction error (mean $\pm$ std) of different variants of our model on medical datasets. The variants in the top row do not leverage physiological variables, whereas the variants in the second row incorporate information about gender and sleep stages. The sleep stages are predicted from breathing (i.e., they do not need to be available as inputs). The table shows that oxygen prediction errors are relatively small and comparable to consumer pulse oximeters, which have an average error that ranges from 0.4\% to 3.5\% ~\citep{lipnick2016accuracy}.}
\label{tab:res-main}
\begin{tabular}{c|c||c|c|c||c}
\toprule
% \hline
\multicolumn{1}{l|}{}                                                        & Model                           & SHHS & MESA & MrOS & Overall              \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o\\Physiological\\Variables\end{tabular}} & Linear Regression   & 1.86 $\pm$ 1.72          & 1.73 $\pm$ 1.73          & 1.87 $\pm$ 1.69          & 1.81 $\pm$ 1.72          \\ 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o Physiological Variables\end{tabular}} & CNN   & 1.72 $\pm$ 0.94          & 1.62 $\pm$ 0.83          & 1.77 $\pm$ 0.86          & 1.73 $\pm$ 0.87          \\ 
& CNN-RNN  & 1.70 $\pm$ 0.92 & 1.56 $\pm$ 0.88  & 1.76 $\pm$ 0.87  & 1.67 $\pm$ 0.87  \\
% & CNN-RNN \cite{zhao2017learning} & - & - & - & -  \\
  & BERT-UNet       & 1.67 $\pm$ 0.92 & 1.55 $\pm$ 0.89  & 1.75 $\pm$ 0.87 & 1.64 $\pm$ 0.88 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}with Physiological Variables\end{tabular}}    & BERT-UNet + VarAug & 1.65 $\pm$ 0.89 & 1.51 $\pm$ 0.82 & 1.68 $\pm$ 0.83 & 1.61 $\pm$ 0.85          \\
% & BERT-UNet +PCGrad  & 1.73 $\pm$ 1.56 & 1.63 $\pm$ 1.57          & 1.70 $\pm$ 1.53          & 1.69 $\pm$ 1.51          \\ 
& \textbf{BERT-UNet + GNP} & \textbf{1.61 $\pm$ 0.87} & \textbf{1.50 $\pm$ 0.83} & \textbf{1.65 $\pm$ 0.79} & \textbf{1.58 $\pm$ 0.83} \\ 
% \hline
\bottomrule
\end{tabular}
% \vspace{-4mm}
% \caption{Prediction error (mean $\pm$ std) of different variants of our model on medical datasets. The variants in the top row do not leverage health variables, whereas the variants in the second row incorporate information about gender and sleep stages. The sleep stages are predicted from breathing (i.e., they do not need to be available as inputs). The table shows that oxygen prediction errors are relatively small and comparable to consumer pulse oximeters, which have an average error that ranges from 0.4\% to 3.5\% ~\citep{lipnick2016accuracy}.}

\end{table*}


%\begin{table}[] 
%\caption{Prediction error of different models on three medical datasets. \yc{The values are from the best checkpoint instead of the newest checkpoint.}}
%\label{tab:res-main}
%\footnotesize
%\centering
%\begin{tabular}{c|ccc|ccc|ccc}
%\toprule
%Model & \multicolumn{3}{c|}{SHHS} & \multicolumn{3}{c|}{MESA} & \multicolumn{3}{c}{MROS} \\ \hline
%     & $<$92 & $\geq$92 & All      & $<$92 & $\geq$92 & All     & $<$92 & $\geq$92 & All     \\
%Single-Head & 4.2 & 1.25 & 1.61 & 4.47 & 1.19 & 1.49 & 3.74 & 1.31 & 1.7 \\
%Multi-Task & \textbf{3.93} & 1.32 & 1.62 & 4.41 & 1.19 & 1.48 & 3.52 & \textbf{1.3} & 1.66 \\
%PCGrad-Adapted & 4.01 & 1.28 & 1.61 & \textbf{4.25} & 1.2 & 1.48 & 3.56 & 1.31 & 1.67 \\
%Multi-Headed & 3.96 & \textbf{1.25} & \textbf{1.58} & 4.37 & \textbf{1.18} & \textbf{1.47} & \textbf{3.42} & 1.31 & \textbf{1.6} \\
%\bottomrule
%\end{tabular}
% \end{table}


==> source/table/main_result.tex <==
\begin{table*}[]
\caption{Prediction error (mean $\pm$ std) of different models on three medical datasets. The linear regression model takes the hand-crafted breathing features proposed by \cite{picard2001toward}. The CNN-RNN and PCGrad models are adapted for the oxygen prediction task. (See models details in Sec.~\ref{sec:models}).}
% \caption{\yy{Prediction error (mean $\pm$ std) of different models trained on all three medical datasets and test on each dataset and the overall dataset. The linear regression model takes the hand-crafted features for respiration signals proposed by \cite{picard2001toward}. The CNN-RNN, PCGrad models are adapted from original papers to our oxygen saturation prediction task. (Models details are described in Sec.~\ref{sec:models}). } }
\label{tab:res-main}
\centering
\begin{tabular}{c|c||c|c|c||c}
\toprule
% \hline
\multicolumn{1}{l|}{}                                                        & Model                           & SHHS & MESA & MrOS & Overall              \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o\\Physiological\\Variables\end{tabular}} & Linear Regression \cite{picard2001toward}  & 1.86 $\pm$ 1.72          & 1.73 $\pm$ 1.73          & 1.87 $\pm$ 1.69          & 1.81 $\pm$ 1.72          \\ 
& CNN-RNN \cite{zhao2017learning} & 1.68 $\pm$ 1.56 & 1.57 $\pm$ 1.56  & 1.72 $\pm$ 1.50  & 1.65 $\pm$ 1.55  \\
% & CNN-RNN \cite{zhao2017learning} & - & - & - & -  \\
  & \textbf{BERT-UNet (Ours)}       & \textbf{1.63 $\pm$ 1.51} & \textbf{1.56 $\pm$ 1.55} & \textbf{1.70 $\pm$ 1.50} & \textbf{1.62 $\pm$ 1.48} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}with\\Physiological\\Variables\end{tabular}}    & BERT-UNet + VarAug & 1.62 $\pm$ 1.50 & 1.52 $\pm$ 1.52 & 1.62 $\pm$ 1.48 & 1.58 $\pm$ 1.47          \\
& BERT-UNet +PCGrad \cite{PCGrad}  & 1.73 $\pm$ 1.56 & 1.63 $\pm$ 1.57          & 1.70 $\pm$ 1.53          & 1.69 $\pm$ 1.51          \\ 
& \textbf{BERT-UNet + GNP (Ours)} & \textbf{1.58 $\pm$ 1.47} & \textbf{1.50 $\pm$ 1.49} & \textbf{1.61 $\pm$ 1.42} & \textbf{1.55 $\pm$ 1.43} \\ 
% \hline
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table*}


==> source/table/sidebyside_umass_comapre.tex <==
\vspace{-1mm}
\begin{table}[t!]
  \begin{minipage}{.42\linewidth}
    \centering
        \caption{Results on the RF dataset.}
        \label{tab:umass}
        \vspace{-1mm}
        \resizebox{0.95\textwidth}{!}{

        \begin{tabular}{c||p{5mm}p{5mm}m{9mm}}
        \toprule
        Model & Corr$^\uparrow$  & MAE$^\downarrow$ & RMSE$^\downarrow$\\
        \hline
        CNN    & 0.45 & 1.65 & 1.73    \\ 
        CNN-RNN  & 0.49 & 1.85 & 1.93  \\
        BERT-UNet  & 0.48 &  1.49 & 1.58 \\ 
        \hline
        BERT-UNet + VarAug & 0.49 & 1.49 & 1.59 \\
        Gated BERT-UNet & \textbf{0.52} & \textbf{1.32} & \textbf{1.54}\\ 
        \bottomrule
        \end{tabular}
        }
  \end{minipage}%
  \hfill
  \begin{minipage}{.56\linewidth}
        \caption{Comparison of previous state-of-the-art oxygen monitoring methods with our \textit{Gated BERT-UNet}.} \label{tab:compare_w_previous_work}
        % \vspace{-0.5mm}

        
        \resizebox{0.95\textwidth}{!}{

        \begin{tabular}{c||p{5mm}p{5mm}p{9mm}|c}
        \toprule
        % \hline
        % \citealp{ding2018measuring}
        Method & Corr$^\uparrow$   &  MAE$^\downarrow$ & RMSE$^\downarrow$ & Contactless    \\ 
        \hline
        Ding et al. 2018  & 0.26 &  2.43 & 2.85 & No  \\ 
        % \hline
        Mathew et al. 2021  & 0.46  & 1.97 & 2.16 & Yes \\ 
        % \hline
        Ours  & \textbf{0.52} &  \textbf{1.32} & \textbf{1.54} & Yes   \\
        \bottomrule
        \end{tabular}
        }
  \end{minipage}
  \vspace{-2mm}
\end{table}


==> source/table/umass-result.tex <==
% %%%%% two column version %%%%
% \begin{table*}[thb] 
% \centering
% \caption{Prediction error for the RF dataset using BB-respiration signals or RF-respiration signals.}
% \vspace{0.1in}
% \label{tab:umass}
% \begin{tabular}{cccc|cccc}
% \toprule
% \multicolumn{4}{c|}{BB-respiration signals} & \multicolumn{4}{c}{RF-respiration signals} \\ \hline
% Awake & Sleep & REM & All & Awake & Sleep & REM & All \\ \hline
% % 1.37  & 1.30  & 1.27 & 1.30 & 1.65 & 1.24 & 1.35 & 1.28 \\
% % \footnotesize
% 1.37 $\pm$ 1.19 & \footnotesize 1.30 $\pm$ 1.28 & \footnotesize 1.27 $\pm$ 1.14 & \footnotesize 1.30 $\pm$ 1.13 & \footnotesize 1.65 $\pm$ 1.46 & \footnotesize 1.24 $\pm$ 0.98 & \footnotesize 1.35 $\pm$ 1.04 & \footnotesize 1.28 $\pm$ 1.04 \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \vspace{-0.1in}

%%%%% single column version %%%%
% \begin{table}[ht!]
% \small
% \centering
% \caption{Prediction error for the RF dataset. The line marked as RF refers to  oxygen prediction based on the RF signals collected using a radio device. The line marked as BB refers to oxygen prediction based on the signal collected from the same subjects using a breathing belt. }
% \label{tab:umass}
% \begin{tabular}{c|cccc} 
% \toprule
% & Awake & Sleep & REM & All  \\ \hline
% RF & 1.65 $\pm$ 1.46 & 1.24 $\pm$ 0.98 & 1.35 $\pm$ 1.04 & 1.28 $\pm$ 1.04 \\
% BB & 1.37 $\pm$ 1.19 & 1.30 $\pm$ 1.28 & 1.27 $\pm$ 1.14 & 1.30 $\pm$ 1.13 \\ 
% \bottomrule
% \end{tabular}
% \end{table}
% \vspace{-4mm}

%%%%%% with comparing results %%%%%%%%
% \begin{table}[t!]
% \small
% \centering

% \caption{Prediction error for the RF datasets. The table shows similar patterns to those in Table 1, and equally small errors. }
% \label{tab:umass}

% \begin{tabular}{c|c||c|c||c}
% \toprule
% % \hline
% \multicolumn{1}{l|}{}                                                        & Model                           & UMass & MGH  & Overall              \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o Physiological Variables\end{tabular}} & CNN   & 1.46 $\pm$ 1.35 & 1.83 $\pm$ 1.45 &  1.75 $\pm$ 1.40     \\ 
% % \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o\\Physiological\\Variables\end{tabular}} & CNN   & 1.86 $\pm$ 1.72          & 1.73 $\pm$ 1.73          & 1.87 $\pm$ 1.69          & 1.81 $\pm$ 1.72          \\ 
% & CNN-RNN  &  1.43 $\pm$ 1.01 & 1.62 $\pm$ 1.19 &  1.58 $\pm$ 1.12   \\
% % & CNN-RNN \cite{zhao2017learning} & - & - & - & -  \\
%   & \textbf{BERT-UNet}  &  1.33 $\pm$ 0.98   & 1.51 $\pm$ 1.55 &   1.38 $\pm$ 1.14 \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}with Physiological Variables\end{tabular}} & BERT-UNet + VarAug & 1.41 $\pm$ 1.08  & 1.37 $\pm$ 1.27  & 1.39 $\pm$ 1.12 \\
% % & BERT-UNet +PCGrad & 1.33 $\pm$ 0.96 &   &  \\ 
% & \textbf{BERT-UNet + GNP} & 1.30 $\pm$ 1.03 & 1.34 $\pm$ 1.26 & 1.33 $\pm$ 1.14 \\ 
% % \hline
% \bottomrule
% \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% two column
% \begin{table*}[t!]
% \small
% \centering
% \caption{Prediction error for the RF dataset.}
% \label{tab:umass}
% \begin{tabular}{c|c||c|c||c}
% \toprule
% \multicolumn{1}{l|}{}                                                        & Model                           & MGH & UMass  & Overall              \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}w/o Physiological Variables\end{tabular}} & CNN   & 1.73 $\pm$ 0.50 & 1.72 $\pm$ 0.45 &  1.73 $\pm$ 0.48     \\ 
% & CNN-RNN  &  1.53 $\pm$ 0.33 & 1.35 $\pm$ 0.60 &  1.38 $\pm$ 0.54   \\
%   & BERT-UNet  &  1.52 $\pm$ 0.49   & 1.34 $\pm$ 0.60 &   1.37 $\pm$ 0.58 \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}with Physiological Variables\end{tabular}} & BERT-UNet + VarAug & 1.38 $\pm$ 0.43 & 1.39 $\pm$ 0.66 & 1.39 $\pm$ 0.61 \\
% & \textbf{BERT-UNet + GNP} & \textbf{1.36 $\pm$ 0.37} & \textbf{1.31 $\pm$ 0.76} & \textbf{1.32 $\pm$ 0.70} \\ 
% \bottomrule
% \end{tabular}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% single column
\begin{table}[t!]
\small
\centering

\caption{Performances of model variants on the RF dataset.}
\label{tab:umass}
\vspace{-2mm}
\begin{tabular}{c||ccc}
\toprule
Model & Corr$^\uparrow$  & MAE$^\downarrow$ & RMSE$^\downarrow$\\
\hline
CNN    & 0.45 & 1.65 & 1.73    \\ 
CNN-RNN  & 0.49 & 1.85 & 1.93  \\
BERT-UNet  & 0.48 &  1.49 & 1.58 \\ 
\hline
BERT-UNet + VarAug & 0.49 & 1.49 & 1.59 \\
Gated BERT-UNet & \textbf{0.52} & \textbf{1.32} & \textbf{1.54}\\ 
\bottomrule
\end{tabular}
\end{table}


==> source/table/umass_result_old.tex <==
% %%%%% two column version %%%%
% \begin{table*}[thb] 
% \centering
% \caption{Prediction error for the RF dataset using BB-respiration signals or RF-respiration signals.}
% \vspace{0.1in}
% \label{tab:umass}
% \begin{tabular}{cccc|cccc}
% \toprule
% \multicolumn{4}{c|}{BB-respiration signals} & \multicolumn{4}{c}{RF-respiration signals} \\ \hline
% Awake & Sleep & REM & All & Awake & Sleep & REM & All \\ \hline
% % 1.37  & 1.30  & 1.27 & 1.30 & 1.65 & 1.24 & 1.35 & 1.28 \\
% % \footnotesize
% 1.37 $\pm$ 1.19 & \footnotesize 1.30 $\pm$ 1.28 & \footnotesize 1.27 $\pm$ 1.14 & \footnotesize 1.30 $\pm$ 1.13 & \footnotesize 1.65 $\pm$ 1.46 & \footnotesize 1.24 $\pm$ 0.98 & \footnotesize 1.35 $\pm$ 1.04 & \footnotesize 1.28 $\pm$ 1.04 \\
% \bottomrule
% \end{tabular}
% \end{table*}
% \vspace{-0.1in}

%%%%% single column version %%%%
\begin{table}[ht!]
\small
\centering
\caption{Prediction error for the RF dataset. The line marked as RF refers to  oxygen prediction based on the RF signals collected using a radio device. The line marked as BB refers to oxygen prediction based on the signal collected from the same subjects using a breathing belt. }
\label{tab:umass}
\begin{tabular}{c|cccc} 
\toprule
& Awake & Sleep & REM & All  \\ \hline
RF & 1.65 $\pm$ 1.46 & 1.24 $\pm$ 0.98 & 1.35 $\pm$ 1.04 & 1.28 $\pm$ 1.04 \\
BB & 1.37 $\pm$ 1.19 & 1.30 $\pm$ 1.28 & 1.27 $\pm$ 1.14 & 1.30 $\pm$ 1.13 \\ 
\bottomrule
\end{tabular}
\end{table}
% \vspace{-4mm}


%%%%% floating version %%%%
% \begin{table*}[] 
% \centering
% \caption{Prediction error for the RF dataset using \yy{BB-respiration signals} or \yy{RF-respiration signals}.}
% \label{tab:umass}
% \begin{tabular}{c|c|c|c}
% \toprule
% \multicolumn{4}{c}{Breathing Belt} \\ \hline
% Awake & Sleep & REM & All  \\ \hline
% 1.37 $\pm$ 1.19 & 1.30 $\pm$ 1.28 & 1.27 $\pm$ 1.14 & 1.30 $\pm$ 1.13 \\ \toprule
%  \multicolumn{4}{c}{Radio-Frequency} \\ \hline
% Awake & Sleep & REM & All  \\ \hline
% 1.65 $\pm$ 1.46 & 1.24 $\pm$ 0.98 & 1.35 $\pm$ 1.04 & 1.28 $\pm$ 1.04 \\
% \bottomrule
% \end{tabular}
% \end{table*}

